CQS: A Formally-Verified Framework for Fair and Abortable Synchronization

Writing concurrent code that is both correct and efficient is notoriously difficult. Thus, programmers often prefer to use synchronization abstractions, which render code simpler and easier to reason about. Despite a wealth of work on this topic, there is still a gap between the rich semantics provided by synchronization abstractions in modern programming languages -- specifically, \emph{fair} FIFO ordering of synchronization requests and support for \emph{abortable} operations -- and frameworks for implementing it correctly and efficiently. Supporting such semantics is critical given the rising popularity of constructs for asynchronous programming, such as coroutines, which abort frequently and are cheaper to suspend and resume compared to native threads. This paper introduces a new framework called \texttt{CancellableQueueSynchronizer} (CQS), which enables simple yet efficient implementations of a wide range of fair and abortable synchronization primitives: mutexes, semaphores, barriers, count-down latches, and blocking pools. Our main contribution is algorithmic, as implementing both fairness and abortability efficiently at this level of generality is non-trivial. Importantly, all our algorithms, including the CQS framework and the primitives built on top of it, come with \emph{formal proofs} in the Iris framework for Coq for many of their properties. These proofs are modular, so it is easy to show correctness for new primitives implemented on top of CQS. From a practical perspective, implementation of CQS for native threads on the JVM significantly improves Java's \texttt{AbstractQueuedSynchronizer}, the only practical abstraction offering similar semantics. In sum, \texttt{CancellableQueueSynchronizer} is the first framework to combine expressiveness with formal guarantees and solid practical performance.

==> algos/barrier.tex <==
\section{The Barrier Implementation}\label{sec:barrier}
We present the algorithms developed on the top of CQS in order of increasing complexity. Starting with the barrier in this section, we present a new count-down-latch algorithm in Section~\ref{sec:count-down-latch}, several semaphore algorithms in Section~\ref{sec:semaphore}, and then finish by presenting blocking pools in Section~\ref{sec:pool}. 

One of the synchronization abstractions that is simple but widely used is a \emph{barrier}, which allows a set of parallel operations to wait until all of them reach a common barrier point via the provided \texttt{arrive()} operation. Our CQS-based implementation is straightforward: it maintains a counter of threads that arrived and increments it in the beginning of the \texttt{arrive()} operation. The last operation resumes all those who previously arrived.

Once the last thread arrives, all the waiters should be resumed. However, if any of these waiters becomes cancelled, the barrier contract is violated {---} fewer waiters will be resumed and break the barrier. Unfortunately, solving this problem would require an ability to \emph{atomically} resume a set of waiters (so either all the waiters are resumed or none), but no real system provides such a primitive.
Thus, similarly to the barrier implementation in Java, we do not support cancellation for barriers. However, instead of breaking the barrier when a thread is cancelled, we ignore cancellations. The intuition behind this design is that even if a waiter has been cancelled, it has successfully reached the barrier point and should not block the other parties from continuing.

\subsection{Algorithm}
Listing~\ref{listing:barrier} presents an algorithm for barrier. We use \sqs{} to maintain a set of waiting \texttt{arrive()}-s, resuming them in an asynchronous mode, so neither \texttt{suspend()} nor \texttt{resume(..)} fails.
The logical state of barrier is represented with the \texttt{remaining} counter, which indicates the remaining number of parties that should arrive at this barrier point. 

The \texttt{arrive()} implementation is straightforward: it atomically decrements the number of remaining parties at line~\ref{line:barrier_faa} and either suspends if there are more parties to wait (line~\ref{line:barrier_susp}) or resumes all waiting parties if this is the last one (line~\ref{line:barrier_resume}). 
% It also checks the number of \texttt{arrive()} calls that do not exceed the specified number of parties, see line~\ref{line:barrier_check}.
It is possible for \texttt{resume(..)} at line~\ref{line:barrier_resume} to be called before the corresponding \texttt{suspend()} at line~\ref{line:barrier_susp}. In this case, CQS puts \texttt{Unit} into the cell in \texttt{resume(..)}, and the delayed \texttt{suspend()} observes the value in the cell and finishes without actual suspension.


\begin{figureAsListingWide}
\begin{minipage}[t]{0.53\textwidth}
\begin{lstlisting} 
val cqs = CancellableQueueSynchronizer<Unit>(
  resumeMode = ASYNC
)

// Init with the number of parties to expect
var remaining: Int = parties #\label{line:barrier_remaining}# 
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.44\textwidth}
\begin{lstlisting}[firstnumber=6]
fun arrive(): Future<Unit> {
  r := FAA(&remaining, -1) #\label{line:barrier_faa}#
  if r > 1: return cqs.suspend() #\label{line:barrier_susp}#
  repeat(parties - 1) { cqs.resume(Unit) } #\label{line:barrier_resume}#
  return ImmediateResult(Unit)
}
\end{lstlisting}
\end{minipage}
\caption{Barrier algorithm via \sqs{}. Like the standard Java library implementation, it does not support cancellation since it would require a practically unavailable ability to resume multiple waiters atomically.}
\label{listing:barrier}
\end{figureAsListingWide}

% \subsection{Progress Guarantee}
% Since our implementation does not support cancellation and the asynchronous resumption mode is used, it is guaranteed that both \texttt{suspend()} and \texttt{resume(..)} on \sqs{} are wait-free. The rest of the \texttt{arrive()} operation is also wait-free, which should be obvious from the code. Therefore, our implementation guarantees wait-freedom.

% \subsection{Correctness}
% \input{proofs/barrier}

\subsection{Evaluation}

\paragraph{Environment.}
All the algorithms presented in this paper are implemented in Kotlin for JVM, using Java threads as waiters.


% \begin{wrapfigure}{r}{0.39\textwidth}
% \vspace{-2em}
\begin{lstlisting}[
  caption={Barrier benchmark.},
  label={listing:barrier_bench},
  numbers=none
]
fun benchmark(threads: Int, work: Int) {
 parallel(threads) {
 #\indentrule#  for i in 1..OPERATIONS:
 #\indentrule#  #\indentrule#  @barrier[i].arrive() @
 #\indentrule#  #\indentrule#  @doGeomDistributedWork(mean = work)@
 }
}
\end{lstlisting}
% \vspace{-1.8em}
% \end{wrapfigure}

\paragraph{Benchmark.}
We compared the \sqs{}-based barrier implementation with the standard one available in Java. The experiment is organized in the following way. Each of the threads performs barrier point synchronizations following by some uncontended work, the size of which is geometrically distributed with a constant mean. This process is repeated a constant number of times. 
We consider each \texttt{arrive()} with the additional work as an operation and count the average time required for it. Thus, without any synchronization, it is expected to decrease linearly with increasing the number of threads. See the pseudo-code of this benchmark in Listing~\ref{listing:barrier_bench}.
%
In practice, we measure the total invocation time of the \texttt{benchmark(..)} function and divide it by $\mathtt{OPERATIONS} \times \mathtt{threads}$ to get the average time of a single operation, which is highlighted with yellow.


% \begin{wrapfigure}{r}{0.37\textwidth}
% \vspace{-1.8em}
\begin{lstlisting}[
  caption={Barrier via spin-waiting.},
  label={listing:barrier_counter},
  numbers=none
]
var remaining = parties
fun arrive() {
  FAA(&remaining, -1) // arrive
  while remaining > 0 {} // spin wait
}
\end{lstlisting}
% \vspace{-1.8em}
% \end{wrapfigure}

Additionally to the Java and CQS-based implementations, we add a simple counter-based solution, which is organized in the same way as ours but performs an active waiting instead of suspension, spinning in a loop until the \texttt{remaining} counter becomes zero. We consider this simple algorithm as a baseline.

% presented in Listing~\ref{listing:barrier_counter} on the right. 
Similarly to ours, it maintains a counter of remaining parties that should reach this barrier point, decrementing it at the beginning of \texttt{arrive()}. However, instead of suspending, it performs an active waiting, 

\paragraph{Results.}
The results are presented in Figure~\ref{fig:barrier_experiment}; we evaluated all three algorithms on various numbers of threads and with three average work sizes {---} $100$ (on the left), $1000$ (in the center), and $10'000$ (on the right) uncontended loop cycles. The graphs show an average time per operation in microseconds, lower is better. 

Since one of the main costs of synchronization is suspending and resuming threads, the counter-based solution is predictably the fastest one. Nevertheless, our \sqs{}-based algorithm (marked as \texttt{CQS}) shows similar performance trends, which is because all the operations are based on \texttt{Fetch-And-Add}-s. In contrast, the solution from the standard concurrency library in Java (marked as \texttt{Java}) shows significantly less scalability {---} we find the reason for such performance degradation in using a mutex under the hood; surprisingly, it does not use \texttt{AbstractQueuedSynchronizer} directly.

As a result, we find our solution on top of \sqs{} simple and efficient, which also provides stable performance.
%Therefore, we would highly recommend using it in practical systems and standard concurrency libraries.  

\begin{figure*}[H]
    \centering
    \includegraphics[width=\textwidth]{plots/barrier.pdf}
    \caption{Evaluation of \sqs{}-based barrier implementation against the standard one available in Java and a simple counter-based solution with active waiting. The plots show average time per operation (\texttt{arrive()} + uncontended work), \textbf{lower is better}.}
    \label{fig:barrier_experiment}
\end{figure*}

==> algos/cdl.tex <==
\section{The Count-Down-Latch}\label{sec:count-down-latch}
The next synchronization primitive we consider is \emph{count-down-latch}, which allows waiting until the specified number of operations are completed.
It is initialized with a given count, and each \texttt{countDown()} invocation decrements the count of remaining operations to be completed. At the same time, the \texttt{await()} operation suspends until the count reaches zero.

\subsection{Algorithm}
The pseudocode of our count-down-latch implementation is presented in Listing~\ref{listing:cdl}. 
Essentially, the latch maintains two counters: \texttt{count} that represents the number of remaining operations (line~\ref{line:cdl_count}), and \texttt{waiters} that stores the number of waiting \texttt{await()}-s (line~\ref{line:cdl_waiters}). 

\paragraph{The \texttt{countDown()} and \texttt{await()} Operations.}
The \texttt{countDown()} function is straightforward: it first decrements the number of remaining operations (line~\ref{line:cdl_cd_inc}), and then resumes the waiting \texttt{await()}-s if the count reached zero (line~\ref{line:cdl_cd_rw}).

Meanwhile, \texttt{await()} checks whether the counter of remaining operations has already reached zero. Since we always decrement \texttt{count} in \texttt{countDown()}, it can become negative if the number of \texttt{countDown()} invocations is greater than the initially specified one. In the current implementation, we allow this behaviour. However, it is also possible to check in \texttt{countDown()} that the counter is still non-negative after the decrement, throwing an exception otherwise.

When \texttt{await()} observes that \texttt{count} is positive, it increments the number of waiters (line~\ref{line:cdl_a_winc}) and suspends (line~\ref{line:cdl_a_susp}). Given that \texttt{resumeWaiters()}, which is invoked by the last \texttt{countDown()}, can be executed concurrently with \texttt{await()}, they should be synchronized. For this purpose, \texttt{resumeWaiters()} sets the \texttt{DONE\_BIT} in the \texttt{waiters} counter, forbidding further suspensions and showing that this count-down-latch has reached zero. Thus, \texttt{await()} checks for this \texttt{DONE\_BIT} before suspension and completes immediately if it is set (line~\ref{line:cdl_a_bitcheck}).

As for \texttt{resumeWaiters()}, it tries to set \texttt{DONE\_BIT} (line~\ref{line:cdl_rw_setbit}) and resume the waiting \texttt{await()}-s, the number of which is stored in \texttt{waiters} at the moment of setting the bit (line~\ref{line:cdl_rw_setbit}). The whole operation is wrapped in an infinite loop and finishes immediately if the bit is already set (line~\ref{line:cdl_rw_bitcheck}), retrying the function from the beginning if the \texttt{CAS} that attempts to set the \texttt{DONE\_BIT} fails (line~\ref{line:cdl_rw_setbit}). 

\paragraph{Cancellation.} 
The simplest way to support cancellation is doing nothing: the algorithm already works with the simple cancellation mode, where \texttt{resume()}-s fail on cancelled cells. In this case, all suspended \texttt{await()}-s increment the number of waiters, while \texttt{resumeWaiters()} tries to resume all of them without checking whether the resumption succeeds or not. However, in this case \texttt{resumeWaiters()} works in a linear time on the total number of \texttt{await()} invocations, including the cancelled ones.

The smart cancellation, in turn, makes it possible to optimize \texttt{resumeWaiters()}, so the number of steps is bounded by the number of non-cancelled \texttt{await()}-s. The \texttt{onCancellation()} function (lines~\ref{line:cdl_onc_start}--\ref{line:cdl_onc_end}) is invoked when a waiter becomes cancelled. It attempts to decrement the number of waiters (line~\ref{line:cdl_onc_decw}), making \texttt{resume()} skip the corresponding cell in the CQS. However, if the \texttt{DONE\_BIT} is already set at the moment of the decrement, a concurrent \texttt{resumeWaiters()} is going to resume this cancelled waiter. Thus, the corresponding \texttt{resume()} should be refused {---} \texttt{onCancellation()} returns \texttt{false} in this case.

\begin{figureAsListingWide}
\begin{minipage}[t]{0.55\textwidth}
\begin{lstlisting} 
val cqs = CancellableQueueSynchronizer<Unit>(
  resumeMode = ASYNC, #\label{line:cdl_sqs_1}#
  cancellationMode = SMART, #\label{line:cdl_sqs_2}#
  onCancellation = ::onCancellation
)
var count: Int = initCount #\label{line:cdl_count}# // init with the given count
var waiters: Int = 0 #\label{line:cdl_waiters}# // no waiters initially
  
fun countDown() {
  r := FAA(&count, -1) // decrement the count #\label{line:cdl_cd_inc}#
  if r <= 1: resumeWaiters() // has it reached zero? #\label{line:cdl_cd_rw}#
}

fun await(): Future<Unit> {
  if count <= 0: return ImmediateResult(Unit)
  w := FAA(&waiters, +1) // inc the number of waiters #\label{line:cdl_a_winc}#
  if w & DONE_BIT != 0: return ImmediateResult(Unit) #\label{line:cdl_a_bitcheck}#
  return cqs.suspend() #\label{line:cdl_a_susp}#
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4\textwidth}
\begin{lstlisting}[firstnumber=20]
fun resumeWaiters() = while(true) {
  w := waiters
  // Is DONE_BIT already set?
  if w & DONE_BIT != 0: return #\label{line:cdl_rw_bitcheck}#
  // Set DONE_BIT and resume waiters
  if CAS(&waiters, w, w | DONE_BIT): #\label{line:cdl_rw_setbit}#
  #\indentrule#  // DONE_BIT is set, resume waiters
  #\indentrule#  repeat(w) { cqs.resume(Unit) } #\label{line:cdl_rw_resume}#
  #\indentrule#  return
}

fun onCancellation(): Bool { #\label{line:cdl_onc_start}#
  // Decrement the number of waiters
  w := FAA(&waiters, -1) #\label{line:cdl_onc_decw}#
  // Succeed if DONE_BIT is not set
  return w & DONE_BIT == 0 #\label{line:cdl_onc_bitcheck}#
} #\label{line:cdl_onc_end}#

const DONE_BIT = 1 << 31
\end{lstlisting}
\end{minipage}
\caption{Count-down-latch implementation on top of \sqs{} with smart cancellation. Changing the cancellation mode to \texttt{SIMPLE} and removing the \texttt{onCancellation()} function produces a correct algorithm with the simple cancellation mode.}
\label{listing:cdl}
\end{figureAsListingWide}

% \sqs{} provides two different cancellation modes, simple and smart; the algorithm below uses the \texttt{SMART\_ASYNC} one. However, changing it to \texttt{SIMPLE} and removing the cancellation handler would keep the algorithm correct but potentially increase the complexity of the invocation of \texttt{countDown()} that reached zero.

% \subsection{Progress Guarantee}
% % Since the asynchronous resumption and the smart cancellation modes are used (lines~\ref{line:cdl_sqs_1}--\ref{line:cdl_sqs_2}), it is guaranteed that both 

% Since \texttt{suspend()} is wait-free and does not fail, the \texttt{await()} operation is obviously wait-free as well. 
% %
% The cancellation, however, is lock-free due to possible segment removing.
% % (see the \texttt{onCancellation()} function at lines~\ref{line:cdl_onc_start}--\ref{line:cdl_onc_end}).

% As for the \texttt{countDown()} operation, it performs \texttt{Fetch-And-Add} at line~\ref{line:cdl_cd_inc} and invokes \texttt{resumeWaiter()} if the count has reached zero at line~\ref{line:cdl_cd_rw}. Thus, the progress guarantee for \texttt{countDown()} is completely dependent on the \texttt{resumeWaiters()} function. Surprisingly, even with the infinite loop wrapper, the number of failed \texttt{CAS}-s to set the \texttt{DONE\_BIT} at line~\ref{line:cdl_rw_setbit} is bounded by the number of concurrent \texttt{await()} invocations, and thus, by the parallelism level in general. When \texttt{resumeWaiters()} is invoked, \texttt{count} has already reached zero, so all the following \texttt{await()} invocations complete immediately and neither change the \texttt{waiters} field nor suspend. As a consequence, \texttt{resume(..)} can skip a bounded number of cancelled cells and is wait-free. In sum, the \texttt{resumeWaiters()} function along with the \texttt{countDown()} operation are wait-free.


\subsection{Evaluation}
Just as we did for the barrier, we implement the presented count-down-latch algorithm in Kotlin for JVM and compared it with the standard implementation from the Java's concurrency package. 

\paragraph{Environment.} The experiments were run on a server with 4 Intel Xeon Gold 6150 (Skylake) sockets; each socket has 18 2.70GHz cores, each of which multiplexes 2 hardware threads, for a total of 144 hardware threads. 

\paragraph{Benchmark.} 
To evaluate different count-down-latch implementations, we consider a workload with a lot of \texttt{countDown()} invocations and a relatively small number of waiters.
%
The pseudo-code of the benchmark is presented in Listing~\ref{listing:cdl_bench}. Similarly to the barrier benchmark, it starts the specified number of threads and simulates the large number of operations executed in parallel; each is simulated with an uncontended geometrically distributed work following by the \texttt{countDown()} invocation. The last \texttt{countDown()} invocation also resumes $100$ waiters.

% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-2em}
\begin{lstlisting}[
  numbers=none,
  caption={Count-down-latch benchmark.},
  label={listing:cdl_bench}
]
fun benchmark(threads: Int, work: Int) {
  parallel(threads) {
  #\indentrule#  repeat(OPERATIONS / threads) {
  #\indentrule#  #\indentrule#  doGeomDistributedWork(mean = work)
  #\indentrule#  #\indentrule#  cdl.countDown()
  #\indentrule#  }
  }
}
\end{lstlisting}
% \vspace{-2em}
% \end{wrapfigure}

Additionally to the standard Java implementation and ours, we add a baseline that does not invoke \texttt{countDown()}. Thus, comparing with this baseline we can measure the overhead caused by the count-down-latch implementation.

\paragraph{Results.}
Figure~\ref{fig:cdl_experiment} shows the evaluation results with different additional work sizes ($50$ uncontended loop cycles on average on the left, $100$ {---} in the center, and $200$ {---} on the right). It is clear that our implementation based on CQS significantly outperforms the standard one from Java by up to $x4$. Comparing to the baseline, it shows the same trend and has a little overhead on the right graph, where the work is $200$ uncontended loop cycles.

\begin{figure*}[H]
    \centering
    \includegraphics[width=\textwidth]{plots/cdl.pdf}
    \caption{Evaluation of \sqs{}-based count-down-latch implementation against the standard one in Java. \textbf{Lower is better.}}
    \label{fig:cdl_experiment}
\end{figure*}

==> algos/pools.tex <==
\section{Blocking Pools}\label{sec:pool}
While the previous algorithms only use \sqs{} for synchronization, it is also possible to develop \emph{communication} primitives on top of it. In this section, we consider simple blocking pool implementations. 

While using resources such as database connections, sockets, etc., it is common to reuse them; that usually requires an efficient and accessible mechanism. The \emph{blocking pool} abstraction maintains a set of elements that can be retrieved to process some operation after which the element is placed back in the pool. Operations \texttt{put(element)} and \texttt{take()} are provided:
\begin{itemize}
 \item \texttt{put(element)} either resumes the first waiting \texttt{take()} operation and passes the element to it, or puts the element into the pool.
 \item \texttt{take()} takes one of the elements from the pool (in an unspecified order), or suspends if it is empty: later 
 \texttt{put(e)} operations resume waiting \texttt{take()}-s in the first-in-first-out order.
\end{itemize}

In this paper, we consider two pool implementations: queue-based and stack-based. Intuitively, the queue-based implementation is faster since it can be built on segments similar to the \sqs{} and uses \texttt{Fetch-And-Add}-s on the contended path. In contrast, the stack-based pool retrieves the last inserted, thus, the ``hottest'', element.
Please note that both algorithms presented in this section are not linearizable and can retrieve elements out-of-order under some races. However, since pools do not guarantee that the stored elements are ordered (one may consider them as bags), these queue and stack-based versions should be considered as pools with specific heuristics.

\subsection{Algorithm}
We start from an abstract solution that does not rely on queues, stacks, or other containers. After that, we provide solutions for queue-based and stack-based pools on top of the abstract pool.

\paragraph{Abstract Blocking Pool.}
Intuitively, the blocking pool contract reminds of a semaphore. It, like the semaphore, transfers resources, with the only difference that semaphore transfers logical non-distinguishable permits while blocking pool works with actual elements. The rest, however, is almost the same. 
%
Listing~\ref{listing:pool_basic} presents the abstract blocking pool implementation on top of \sqs{} with asynchronous resumption and smart cancellation (lines~\ref{line:pools_basic:resumeMode}~and~\ref{line:pools_basic:cancellationMode}). Like in the semaphore, the algorithm maintains the \texttt{size} counter (line~\ref{line:pools_basic:size}), which represents the number of elements in the pool if it is non-negative, and the number of waiters with the minus sign otherwise. 

The \texttt{put(..)} operation increments the \texttt{size} counter first (line~\ref{line:pools_basic:put:inc}), and either resumes the next waiter if the counter was negative (line~\ref{line:pools_basic:put:resume}) or adds the element to the pool structure via \texttt{tryInsert(..)} function if no waiter was there (line~\ref{line:pools_basic:put:tryInsert}). In our design, \texttt{tryInsert(..)} can fail if a racy \texttt{take()} operation comes to the pool between the counter increment and the \texttt{tryInsert(..)} invocation {---} both operations should restart in this case.

The \texttt{take()} operation decrements the \texttt{size} counter first (line~\ref{line:pools_basic:take:dec}), and either tries to retrieve an element from the pool structure via \texttt{tryRetrieve(..)} if the size was positive (lines~\ref{line:pools_basic:take:tryRetrieve0}--\ref{line:pools_basic:take:tryRetrieve1}) or suspends in the \sqs{} if there is no element to retrieve (line~\ref{line:pools_basic:take:suspend}).

As for the cancellation logic, the \texttt{onCancellation()} implementation is identical to the one in semaphore: it increments the \texttt{size} counter (line~\ref{line:pools_basic:onCancellation:inc}) and returns \texttt{true} if the number of waiters was decremented (so the counter was negative) or returns \texttt{false} if there is an upcoming \texttt{resume(..)} that should be refused.
In order to refuse the value, the algorithm tries to insert it back to the pool structure (the \texttt{tryReturnRefusedValue(..)} function is specified at line~\ref{line:pools_basic:tryReturnRefused}), and on its failure a a full \texttt{put(..)} is performed (the \texttt{returnValue(..)} function is specified at line~\ref{line:pools_basic:returnValue}).

In order to complete the pool implementation, we need to specify the \texttt{tryInsert(..)} and \texttt{tryRetrieve()} functions.

\begin{figureAsListingWide}
\begin{minipage}[t]{0.46\textwidth}
\begin{lstlisting} 
val cqs = CancellableQueueSynchronizer<Unit>(
  resumeMode = ASYNC, #\label{line:pools_basic:resumeMode}#
  cancellationMode = SMART, #\label{line:pools_basic:cancellationMode}#
  onCancellation = ::onCancellation,
  tryReturnRefusedValue = ::tryInsert, #\label{line:pools_basic:tryReturnRefused}#
  returnValue = ::put #\label{line:pools_basic:returnValue}#
)
var size: Int = 0 // #\color{Mahogany}$\geq$ 0# => size #\label{line:pools_basic:size}#
                  // < #\color{Mahogany}0# => number of waiters
fun put(element: E) = while (true) {
  s := FAA(&size, 1) // increment the size #\label{line:pools_basic:put:inc}#
  // Is there a waiting `retrieve()`?
  if s < 0:
  #\indentrule#  // Resume the first waiter and complete
  #\indentrule#  cqs.resume(element) #\label{line:pools_basic:put:resume}#
  #\indentrule#  return
  else:
  #\indentrule#  // Try to insert the element. Can fail due
  #\indentrule#  // to a race when a concurrent retrieve() 
  #\indentrule#  // discovered the size increment but the 
  #\indentrule#  // corresponding tryRetrieve() has failed
  #\indentrule#  if tryInsert(element): return #\label{line:pools_basic:put:tryInsert}#
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.51\textwidth}
\begin{lstlisting}[firstnumber=24]
fun take(): Future<T> = while(true) {
  s := FAA(&size, -1) // decrement the size #\label{line:pools_basic:take:dec}#
  if s > 0:
  #\indentrule#  // Try to retrieve an element. Can fail due to
  #\indentrule#  // a race when a concurrent put(e) incremented  
  #\indentrule#  // the size but hasn't inserted the element yet
  #\indentrule#  x := tryRetrieve() #\label{line:pools_basic:take:tryRetrieve0}#
  #\indentrule#  if x != null: return ImmediateResult(x) #\label{line:pools_basic:take:tryRetrieve1}#
  else:
  #\indentrule#  return cqs.suspend() // no elements, suspend #\label{line:pools_basic:take:suspend}#
}

fun onCancellation(): Bool {
  s := FAA(&size, 1) #\label{line:pools_basic:onCancellation:inc}#
  // Succeed if the waiter is not going to be 
  // resumed now, refuse the element otherwise
  return s < 0 
}

// tryInsert(e) fails => the paired tryRetrieve()
// should fail as well, and vise versa
fun tryInsert(element: E): Bool
fun tryRetrieve(): E?
\end{lstlisting}
\end{minipage}
\caption{Abstract blocking pool implementation that maintains the \texttt{size} counter of available elements (if positive) or waiting retrievals (if negative). All the waiting \texttt{take()} operations are processed in first-in-first-out order, while the pool itself can use any concurrent data structure under the hood. In Listing~\ref{listing:pool_stack_and_queue}, we present two solutions: based on a concurrent stack, which returns the ``hottest'' element, and based on a queue, which is relatively more efficient.}
\label{listing:pool_basic}
\end{figureAsListingWide}


\paragraph{Queue-Based Pool.} 
The pool with a queue under the hood is shown on the left side of Listing~\ref{listing:pool_stack_and_queue}. Our implementation is based on an infinite array (line~\ref{line:poolq:infarr}), which can be emulated in a way similar to how it is done in \sqs{}.

The \texttt{tryInsertQueue(..)} (we added \texttt{Queue} and \texttt{Stack} suffixes to distinguish the implementations) operation increments its \texttt{insertIdx} counter (line~\ref{line:poolq:insert:inc}) and tries to atomically change the corresponding slot in the infinite array from \texttt{null} to the given element via \texttt{CAS} (line~\ref{line:poolq:insert:cas}). If this \texttt{CAS} fails, it means that a concurrent \texttt{tryRetrieveQueue()}, which already discovered the preceding \texttt{size} increment, came to the same array slot and broke it (line~\ref{line:poolq:retrtieve:cas}) {---} \texttt{tryInsertQueue(..)} returns \texttt{false} in this case.

The \texttt{tryRetrieveQueue()} operation increments its \texttt{retrieveIdx} counter (line~\ref{line:poolq:retrtieve:inc}) and tries to retrieve an element from the corresponding infinite array slot (line~\ref{line:poolq:retrtieve:cas}). If the slot is empty, it breaks it by atomically replacing \texttt{null} with a special token and returns \texttt{false}, causing the paired \texttt{tryInsertQueue(..)} to fail as well (line~\ref{line:poolq:insert:cas}).


\paragraph{Stack-Based Pool.} 
The pool with a classic Treiber stack under the hood is present on the right side of Listing~\ref{listing:pool_stack_and_queue}. To deal with races that happen when \texttt{put(..)}, which has already incremented the \texttt{size} counter but has not inserted the element yet, interferes with a concurrent \texttt{take()} that tries to retrieve it, we use the same approach as breaking slots in the previously discussed queue-based pool. The difference is that, instead of breaking slots, \texttt{tryRetrieveStack()} inserts a ``failed node'' if the stack is empty or contains other failed nodes (lines~\ref{line:pools:retrieve:check}--\ref{line:pools:retrieve:failed}); otherwise, it removes the top node with an element (line~\ref{line:pools:retrieve:normal}). On the opposite side, \texttt{tryInsertStack()} checks that the stack does not have these ``failed nodes'', removing one and failing if they exist (lines~\ref{line:pools:insert:check}--\ref{line:pools:insert:failed}), and otherwise, inserting a node with the specified element (line~\ref{line:pools:insert:normal}). 
This algorithm part is almost the same as the unfair synchronous queue by ??? et al.~\cite{}.


\begin{figureAsListingWide}
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting} 
// The queue is based on an infinite array 
// with two counters for insertions and 
// retrievals. The infinite array can be 
// emulated with a list of segments.
val elementsArray: InfiniteArray<E?> #\label{line:poolq:infarr}#
var insertIdx: Long = 0 #\label{line:poolq:insertIdx}#
var retrtieveIdx: Long = 0 #\label{line:poolq:retrtieveIdx}#

fun tryInsertQueue(element: E): Bool {
  // Get an index for this insertion
  i := FAA(&insertIdx, 1) #\label{line:poolq:insert:inc}#
  // Try to put the element into the slot,
  // fails if it is already broken by a paired
  // retrieval that came to the slot earlier.
  return CAS(&elementsArray[i], null, element) #\label{line:poolq:insert:cas}#
}

fun tryRetrieveQueue(): E? {
  // Get an index for this retrieval
  i := FAA(&retrtieveIdx, 1) #\label{line:poolq:retrtieve:inc}#
  // Replace the slot value with #\color{Mahogany}$\bot$#. 
  // If it was null, the slot becomes broken 
  // and this retrieval attempt fails.
  return GetAndSet(&elementsArray[i], #$\bot$#) #\label{line:poolq:retrtieve:cas}#
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.51\textwidth}
\begin{lstlisting}[firstnumber=26]
class Node(val element: E, next: Node) // stack node
var top: Node? = null // the top node of the stack

fun tryInsertStack(element: E): Bool = while(true) {
  t := top // read the current top node of the stack
  // Does this stack contain failed retrievals?
  if t != null && t.element == #$\bot$#: #\label{line:pools:insert:check}#
  #\indentrule#  // Remove the failed node and return `false`
  #\indentrule#  if CAS(&top, t, t.next): return false #\label{line:pools:insert:failed}#
  else:
  #\indentrule#  // The stack is either empty or stores elements
  #\indentrule#  if CAS(&top, t, Node(element, t)): return true #\label{line:pools:insert:normal}#
}

fun tryRetrieveStack(): E? = while (true) {
  t := top // read the current top node of the stack
  // Does this stack have elements to retrieve?
  if t == null || t.element == #$\bot$#:  #\label{line:pools:retrieve:check}#
  #\indentrule#  // The stack is either empty or contains failed
  #\indentrule#  // retrievals, add one more and return null
  #\indentrule#  if CAS(&top, t, Node(#$\bot$#, t): return null #\label{line:pools:retrieve:failed}#
  else:
  #\indentrule#  // The stack has elements, remove the top one
  #\indentrule#  CAS(&top, t, t.next): return t.element #\label{line:pools:retrieve:normal}#
}
\end{lstlisting}
\end{minipage}
\caption{Blocking pool specializations built on top of the solution in Listing~\ref{listing:pool_basic} with queue (on the left) and stack (on the right) under the hood. Intuitively, the queue-based implementation is faster since it is based on arrays and uses \texttt{Fetch-And-Add}-s on the contended path, while the stack-based pool retrieves the last inserted, thus, the ``hottest'', element.}
\label{listing:pool_stack_and_queue}
\end{figureAsListingWide}

% \subsection{Progress Guarantee}
% First of all, the queue-based pool provides wait-free \texttt{tryInsert(e)} and \texttt{tryRetrieve()} functions, while in the stack-based version they ensure lock-freedom.
% However, additions and removals can interfere in an obstruction-free way due to the slot breaking in the queue-based version and publishing ``failed nodes'' in the stack-based one. Nonetheless, they always complete in a bounded number of steps when all other threads are paused. Therefore, all the operations, including the cancellation that can invoke \texttt{put(..)} are obstruction-free. 

\subsection{Evaluation}
We implement both queue-based and stack-based pools and compare them against the existing \texttt{ArrayBlockingQueue} (both fair and unfair) and \texttt{LinkedBlockingQueue} collections from the standard Java library. It is worth noting that these collections provide linearizability while our pools do not. However, they can be considered as standard solutions for the problem of pools of shared resources.

\paragraph{Environment.} The experiments were run on a server with 4 Intel Xeon Gold 6150 (Skylake) sockets; each socket has 18 2.70GHz cores, each of which multiplexes 2 hardware threads, for a total of 144 hardware threads. 

\paragraph{Benchmark.}
We use the same benchmark as for semaphores presented in Subsection~\ref{subsec:sema_eval}. In short, we run many operations on the specified number of threads with a shared pool of elements. Each operation performs some work ($100$ uncontended loop cycles on average in our experiment) first, then takes an element, performs some other work with this element ($100$ more uncontended loop cycles on average in our experiment), and returns it to the pool at the end. The results with other average work values are omitted but were examined and do not differ significantly.

\paragraph{Results.}
Figure~\ref{fig:pools_experiment} shows the results with the different numbers of shared in the pool elements. First of all, the queue-based version shows better results on larger numbers of elements, which is expected as the queue perform a \texttt{Fetch-And-Add} on the contended path and does not restart an attempt to insert or retrieve an element. 
Compared to the fair \texttt{ArrayBlockingQueue}, both of our implementations are always more performant by up to $x100$ times.

The unfair \texttt{LinkedBlockingQueue} is more scalable than the unfair version of \texttt{ArrayBlockingQueue}, and they slightly outperform our fair implementations on a large number of threads with a small number of shared elements, which is when our solutions suspend a lot. However, both our solutions always outperform these unfair primitives up to $x10$ times starting with the number of shared elements equal $8$, and show the same or better performance on the number of threads up to twice the number of elements when the latter is lower than $8$.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{plots/pools.pdf}
    \caption{Evaluation of the presented queue- and stack-based pool algorithms with various numbers of shared elements against the existing \texttt{ArrayBlockingQueue} (both fair and unfair versions) and \texttt{LinkedBlockingQueue} collections from the standard Java library. \textbf{Lower is better.}}
    \label{fig:pools_experiment}
\end{figure*}

==> algos/semaphore.tex <==
\section{The Semaphore}\label{sec:semaphore}
The barrier and count-down-latch algorithms described above do not actually require waiters to be resumed in FIFO order. However, it is important for some primitives such as mutex or semaphore. While mutex allows at most one thread to be in the critical section, wrapped by \texttt{lock()} and \texttt{unlock()} invocations, semaphore is a generalization of mutex that allows the specified number of threads to enter the critical section. This way, a semaphore parameterized with $K=1$ is a mutex. This section presents a fair semaphore algorithm, which also serves as the one for mutex. 

\subsection{Algorithm}
The semaphore algorithm is similar to the mutex one discussed during the CQS details presentation. The only significant difference is that instead of a single ``unlocked'' state, the counter stores the number of available permits. Listing~\ref{listing:semaphore_async_smart} shows the corresponding pseudocode.

In the presented implementation, we use the asynchronous resumption (line~\ref{line:sema:async}) and the smart cancellation (line~\ref{line:sema:smart}) modes; other variants are omitted and can be easily constructed following by the mutex implementations discussed in Sections~\ref{sec:basic}~and~\ref{sec:abortability}. 
The \texttt{permits} field (line~\ref{line:sema:permits}) stores either the number of permits when positive or $0$, or the number of waiters when negative. Similarly to the mutex algorithm, \texttt{acquire()} decrements this counter and suspends if needed, while \texttt{release()} increments it and resumes the first waiter if required. 

\paragraph{The \texttt{acquire()} Operation.}
First, the \texttt{permits} counter is decremented (line~\ref{line:sema:acquire:dec}). If the counter was positive {---} thus, the number of available permits was positive, {---} the operation has successfully taken a permit and completes immediately (line~\ref{line:sema:acquire:acquired}). Otherwise, no permits are available, so it suspends in the \sqs{} (line~\ref{line:sema:acquire:suspend}).

\paragraph{The \texttt{release()} Operation.}
First, in decrements the \texttt{permits} counter (line~\ref{line:sema:release:inc}). If the counter was non-negative, then no operation is waiting in the CQS, so the permit is successfully returned to the semaphore, and the operation completes. Otherwise, if the counter was negative, the next waiter should be resumed (line~\ref{line:sema:release:resume}).

\paragraph{Cancellation.}
When a waiting \texttt{acquire()} is cancelled, it increments the \texttt{permits} counter (line~\ref{line:sema:onCancellation:inc}). If the counter was negative, this increment successfully decremented the number of waiters, so the cancellation succeeds and \texttt{onCancellation()} returns \texttt{true}. Otherwise, if the counter was non-negative, there already is a concurrent \texttt{release()} that will resume the current waiter eventually. In this case, the corresponding \texttt{resume()} should be refused, and the permit has to be returned back to the semaphore via the \texttt{release()} invocation (this is specified in the CQS initialization at line~\ref{line:sema:returnValue}).

\begin{figureAsListingWide}
\begin{minipage}[t]{0.47\textwidth}
\begin{lstlisting} 
val cqs = CancellableQueueSynchronizer<Unit>(
  cancellationMode = SMART, #\label{line:sema:smart}#
  onCancellation = ::onCancellation
  returnValue = ::release #\label{line:sema:returnValue}#
)
var permits: Int = K // #\color{Mahogany}$\geq$ 0# - number of permits #\label{line:sema:permits}#
                     // < #\color{Mahogany}0# - number of waiters
fun acquire(): Future<Unit> {
  // Either decrement the number of available
  // permits or increment the number of waiters
  p := FAA(&permits, -1) #\label{line:sema:acquire:dec}#
  // Is the permit acquired? 
  if p > 0: return ImmediateResult(Unit) #\label{line:sema:acquire:acquired}#
  // Suspend otherwise
  return cqs.suspend() #\label{line:sema:acquire:suspend}#
}
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\textwidth}
\begin{lstlisting}[firstnumber=19]
fun release() {
  // Either increment the number of available
  // permits or decrement the number of waiters
  p := FAA(&permits, 1) #\label{line:sema:release:inc}#
  // Is there a waiter to be resumed?
  if p < 0: cqs.resume(Unit) #\label{line:sema:release:resume}#
}
fun onCancellation(): Bool {
  // Either increment the number of available
  // permits or decrement the number of waiters.
  p := FAA(&permits, 1) #\label{line:sema:onCancellation:inc}#
  // If the number of waiters was decremented,
  // the cancellation is completed, return `true`.
  // Otherwise, there is a `release()` that is 
  // going to resume this waiter, refuse it.
  return p < 0
}
\end{lstlisting}
\end{minipage}
\caption{Semaphore implementation on the top of \sqs{} with asynchronous resumption mode and smart cancellation. The initial number of permits is $K$. In order to use the synchronous resumption mode, both \texttt{acquire()} and \texttt{release()} should restart when \texttt{suspend()} and \texttt{resume(..)} fail. Thus, it becomes possible to implement an additional \texttt{tryAcquire()} operation that attempts to take a permit if it is available {---} it simply decrements the \texttt{permits} counter if it is positive or fails otherwise.}
\label{listing:semaphore_async_smart}
\end{figureAsListingWide}

% \subsection{Progress Guarantee}

% Consider the case where no cancellation happened during the execution. In this case, both \texttt{suspend()} and \texttt{resume(..)} are wait-free, so \texttt{acquire()} and \texttt{release()} are also wait-free. However, when synchronous resumption is used, concurrent \texttt{suspend()} and \texttt{resume(..)} can lead to each other's fails. Therefore, with synchronous resumption, the operations may restart, so only obstruction-freedom is guaranteed.

% Cancellation weakens the progress guarantees. With asynchronous resumption, \texttt{resume(..)} is only lock-free since there can be an infinite sequence of \texttt{suspend()}-s followed by successful cancellations, so any given \texttt{resume(..)} may not finish while the system makes progress. Similarly, the cancellation part is lock-free because it can invoke \texttt{resume(..)}.
% With the synchronous resumption, the cancellation part is always wait-free since it never invokes \texttt{resume(..)} while the \texttt{resume(..)} operation itself is blocking.


\subsection{Evaluation}\label{subsec:sema_eval}

We implemented the presented semaphore with both asynchronous and synchronous resumption modes for Java and Kotlin Coroutines. This way, we compare against the standard semaphore and mutex algorithms from the standard Java library and the current mutex implementation in Kotlin Coroutines.
We also compare against unfair implementations of mutex and semaphore in Java.

\paragraph{Environment.} The experiments were run on a server with 4 Intel Xeon Gold 6150 (Skylake) sockets; each socket has 18 2.70GHz cores, each of which multiplexes 2 hardware threads, for a total of 144 hardware threads. 

\paragraph{Benchmark.}
Consider the workload of many operations to be executed by the specified number of threads with the restricted parallelism level via semaphore. This way, each operation invocation is wrapped with the \texttt{acquire()-release()} pair. When the parallelism level equals $1$, the semaphore is de facto a mutex, so we can compare our semaphore against other mutex algorithms. As before, the operations are simulated with uncontended geometrically distributed work. Besides, we perform additional work before acquiring a permit; thus, simulating a preparation phase for the guarded by semaphore operation.
We used $100$ uncontended loop cycles on average for both the works, so that \texttt{workOut = workIn = 100}. The results with other average work sizes are omitted but were examined and change the results insignificantly.
The pseudocode of this benchmark is presented in Listing~\ref{listing:sema_bench}.

% \begin{wrapfigure}{r}{0.43\textwidth}
% \vspace{-2em}
\begin{lstlisting}[
  numbers=none,
  caption={Semaphore and mutex benchmark.},
  label={listing:sema_bench}
]
fun benchmark(threads: Int, workIn: Int, 
                            workOut: Int) {
  parallel(threads) {
  #\indentrule#  repeat(OPERATIONS / threads) {
  #\indentrule#  #\indentrule#  doGeomDistributedWork(mean = workOut)
  #\indentrule#  #\indentrule#  s.acquire()
  #\indentrule#  #\indentrule#  doGeomDistributedWork(mean = workIn)
  #\indentrule#  #\indentrule#  s.release()
  #\indentrule#  }
  }
}
\end{lstlisting}
% \vspace{-2em}
% \end{wrapfigure}

\paragraph{Results on Java.}
The results against both fair and unfair versions of the standard \texttt{ReentrantLock} and \texttt{Semaphore} primitives in Java plus the classic CLH and MCS locks are shown in Figure~\ref{fig:sema}. 
In the mutex scenario, all the fair algorithms show the same performance, while the unfair mutex and semaphore versions are predictably faster. 

In the semaphore scenario, our solutions outperform both fair and unfair Java implementations when the number of threads does not exceed the number of permits (thus, suspensions do not happen). With increasing the number of semaphore permits, our algorithms almost reach the unfair version and significantly outperform the fair version. 
In particular, our semaphore implementation outperforms the standard fair algorithm in Java up to \texttt{4x} when the number of threads does not exceed the number of permits and up to \texttt{90x} in a highly-contended scenario. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{plots/sema.pdf}
    \caption{Evaluation of \sqs{}-based semaphore implementations compared to the standard ones in Java, including the unfair variants. In addition, we compare our semaphores against the standard lock implementation in Java, including the unfair variant, and the classic CLH and MCS mutexes. Notice that the Y-axis is logarithmically scaled. \textbf{Lower is better.}}
    \label{fig:sema}
\end{figure*}

\paragraph{Results on Kotlin Coroutines.}
At the point of writing this paper, only the mutex implementation was provided by the Kotlin Coroutines library.
\footnote{The existing semaphore implementation was added by the authors as a part of the project on \sqs{}. Please, do not check the authors of the corresponding commits to keep the anonymity of this submission.}
Thus, we evaluate our semaphore algorithm as a mutex one. 
Unlike the experiment on Java, we create multiple coroutines (the number of coroutines is typically much larger than the number of scheduler threads) and execute them on a scheduler with the specified number of threads.
The works before the acquisition and under the lock are equal to $100$ uncontended loop cycles on average.
Listing~\ref{fig:mtuex_coroutines} shows the speedups of our implementations with the asynchronous (\texttt{CQS Async)} and synchronous (\texttt{CQS Sync}) resumption modes against the existing mutex implementation on $1000$ and $10'000$ coroutines. Here we see that our solution outperforms the existing mutex implementation by $\approx10\%$ on average and up to $40\%$ on certain scenarios.

\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{plots/mutex_coroutines.pdf}
    \caption{Evaluation of the presented semaphore algorithm against the existing mutex implementation in Kotlin Coroutines; here, we show the speedup-s. \textbf{Higher is better.}}
    \label{fig:mtuex_coroutines}
\end{figure*}
